EnCortex: A General, Extensible and Scalable Framework for Decision Management in New-age Energy Systems

With increased global warming, there has been a significant emphasis to replace fossil fuel-dependent energy sources with clean, renewable sources. These new-age energy systems are becoming more complex with an increasing proportion of renewable energy sources (like solar and wind), energy storage systems (like batteries), and demand side control in the mix. Most new-age sources being highly dependent on weather and climate conditions bring about high variability and uncertainty. Energy operators rely on such uncertain data to make different planning and operations decisions periodically, and sometimes in real-time, to maintain the grid stability and optimize their objectives (cost savings, carbon footprint, etc.). Hitherto, operators mostly rely on domain knowledge, heuristics, or solve point problems to take decisions. These approaches fall short because of their specific assumptions and limitations. Further, there is a lack of a unified framework for both research and production environments at scale. In this paper, we propose EnCortex to address these challenges. EnCortex provides a general, easy-to-use, extensible, and scalable energy decision framework that enables operators to plan, build and execute their real-world scenarios efficiently. We show that using EnCortex, we can define and compose complex new-age scenarios, owing to industry-standard abstractions of energy entities and the modularity of the framework. EnCortex provides a foundational structure to support several state-of-the-art optimizers with minimal effort. EnCortex supports both quick developments for research prototypes and scaling the solutions to production environments. We demonstrate the utility of EnCortex with three complex new-age real-world scenarios and show that significant cost and carbon footprint savings can be achieved.

==> results.tex <==
\section{Results}
\label{sec:results}
\subsection{Support for Abstractions and Composability}
Table including per scenario types of sources, state spaces, action spaces, number of decisions (like day-ahead vs. intra-day etc.
May be, code snippet to showcase the easy of configuration in config file and composability of including abstractions in scenario 1.

%\input{results/abs_comp}

\subsection{Support for different Optimizers}
\input{results/diff_opt}


Table 1 (Scenario 1)
Scenario 2- Microgrids
MILP vs. Heuristic (scenario 3)

\subsection{Support for uncertainty in different forecasts}
% Combine Tables 2 \& 3 with forecast error margins and effect on savings.
% combining tables 4 \& 5 and show results 6. RL adapting and learning to uncertainty in data.
\input{results/supp_uncert}



\subsection{Support for what-if Analysis and hyper-parameter tuning}
\subsubsection{Degradation cost analysis (Scenario 1)}
With no degradation much faster switching compared to with degradation. Compare against price/carbon on 2nd y axis. Get the results for Fig 13 (verify results) and Fig 14.
Fig \ref{fig:deg_batt_soc}, \ref{fig:deg_cap_vs_degcost},
\ref{fig:deg_cycle_counts},




\subsubsection{Behaviour cloning}
\subsubsection{Pareto intersection for joint optimization}


\subsection{tuning of timesteps/horizon:}
Ref to fig \ref{fig:timeunit_savings} , \ref{fig:timeunit_soc}, \ref{fig:horizon}


% \includegraphics[width=0.85\columnwidth,height=1.5in]{images/figures/timeunit_horizon.png}
% \includegraphics[width=0.85\columnwidth,height=1.5in]{images/figures/timeunit_savings.png}
% \includegraphics[width=0.85\columnwidth,height=1.5in]{}


\subsection{Benchmarking Optimizers}
% Latency support to run different algorithms
% Table in Fig 15 with details on the data (whether the time is for an epoch, full dataset? daset size)
% Takeaways- 
% Supporting both traditional and NN optimizers. Offline or online - latency need to take into account for online and real-time algorithms.
Within \pname, the supported optimizers are either exact solvers(MILP), search-based solvers(SA) or learnable optimizers(DQN-RL). These optimizers have two kinds of latency: (i) Online latency which measures speed of execution runtime and (ii) Offline latency, that measures time to complete one full episode on the dataset that is required for it to be employed online i.e. training time per episode of DQN-RL. Table \ref{tab:latency} shows the latency of each of the supported optimizers on the EA Scenario. This benchmark provides runtime information that is required when choosing optimizers.

\begin{table}[hbtp]
\caption{Comparing offline and online latencies of different optimizers supported within \pname.}
\begin{tabular}{|c|c|c|}
\hline
Optimizer   & Online Latency(s)                  & Offline Latency(s) \\ \hline
DQN-RL(GPU) & 0.000442 \pm 0.0072 &  1423.5 \pm 23.72  \\ \hline
DQN-RL(CPU) & 0.0066 \pm 0.013    &  1443 \pm 1.5  \\ \hline
MILP        & 0.42576 \pm 0.00315 & \---               \\ \hline
SA          & 195.088 \pm 4.903   & \---               \\ \hline
\end{tabular}
\label{tab:latency}
\end{table}



==> results/abs_comp.tex <==
\begin{table}[]
\centering
\scalebox{0.8}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Scenario                      & Energy Source(E) & Storage (S) & Markets(M) & Consumers(C) & Environment & Max actions(step-wise) \\ \hline
Battery Arbitrage             &\---               & \checkmark        & \xmark      &\---           & Fixed       & S              \\ \hline
Microgrid Optimization        & \checkmark             & \checkmark        & \checkmark      & \checkmark         & Fixed       & S + M          \\ \hline
Market Bidding and Allocation & \checkmark             & \checkmark        & \checkmark       & \checkmark         & Dynamic     & S + M + C      \\ \hline
\end{tabular}
}
\end{table}

==> results/diff_opt.tex <==
\begin{table}[hbtp]
\centering
\caption{Savings across different Optimizers when mean of previous 10 days' actual values are used as forecasts: Takeway: MILP performs better than the black-box optimizers. The best result of DQN is taken across 3 seeds.}
\scalebox{0.9}{
\begin{tabular}{|c|c|c| c|}
\hline
      \textbf{Objective}& \textbf{Algorithm} & \multicolumn{2}{|c|}{\textbf{Savings}} \\\cline{3-4}
     & & Cost & Carbon \\ 
     & &  (in EUR) &  (in gCO2eq)\\ \hline
     & SA & 54593.42 &   -41638.32  \\
     Cost  & DQN & 85177.23 & -82077.83 \\
     Optimization & MILP & 88198.84 & -43539.75  &  \hline
    & SA& -22308.67 &   102544.02 \\
     Carbon  & DQN& -36437.6 & 140219.63\\
     Optimization & MILP& -6016.38 & 163336.50 \\ \hline
          %& MPC&-19566.38 &   \textbf{177255.89}\\\hline
      %MPC& \textbf{96713.35} &   -49087.53\\\hline
\end{tabular}
}
\label{tab:opt_results_battery_arbitrage}
\end{table}

\begin{table}[hbtp]
\caption{Microgrid optimization: Performance of different optimizers to maximize cost savings: Takeaway: MILP performs the best overall}
\begin{tabular}{|l|l|}
\hline
Optimizer & Cost Savings(€) \\ \hline
DQN       & 47325908.25    \\
SA      & 47387310.49    \\
MILP        & \textbf{47388106.27}    \\ \hline
\end{tabular}
\label{tab:opt_microgrid_results}
\end{table}\\

\begin{table}[hbtp]
\begin{tabular}{|l|l|}
\hline
Optimizer & Profit() \\ \hline
Heuristic & Place    \\
MILP      & Place    \\ \hline
\end{tabular}
\caption{Placeholder}
\label{tab:market_results}
\end{table}

==> results/supp_uncert.tex <==
In this part of the section, we explore how our optimizers perform with varying forecasting methods. Specifically, we explore optimizing for cost and carbon savings with MILP and DQN as our optimizers on six forecasting methods, stated in \ref{sec:infra_components}. From Table \ref{tab:milp_dqn_for_forecasts_ba}, we observe two ends of the forecasting error spectrum, where the range of MAE is relatively lower for all forecasting methods for price forecasting as opposed to carbon forecasting, arising from the fact that the time-series of carbon emissions lack seasonality and is often harder to predict, as depicted by the performance of LightGBM and N-BEATS on the dataset. While the DQN-RL optimizer comfortably outperforms MILP in cost savings, it slightly lags behind MILP in carbon savings, likely caused due to the fact that accounting for high uncertainty is a much more difficult task for the DQN-RL optimizer.

% Optimization - MILP vs RL
\begin{table}[h]
\centering
\scalebox{0.8}{
\begin{tabular}{|c|c|c| c|}
\hline
      \textbf{Objective}& \textbf{Algorithm} & \multicolumn{2}{|c|}{\textbf{Savings}} \\\cline{3-4}
     & & Cost & Carbon \\ 
     & &  (in EUR) &  (in gCO2eq)\\ \hline
     Cost  & DQN & \textbf{117727.62} & -59906.70 \\
     Optimization & MILP & 116106.74 & -42720.57  \\ \hline
     Carbon  & DQN& -15347.10 &211594.86\\
     Optimization & MILP& -8687.30 & \textbf{227272.49} \\ \hline
     Joint  & DQN & 81545.06 & 137774.50\\
     Optimization($\alpha=1.115$) &MILP & 74898.32 & \textbf{164751.74} \\ \hline
\end{tabular}
}
\caption{Savings across different Objectives when forecasts are very accurate. Takeaway: Depending on the input forecast data, RL performs better in price-optimization while MILP better in the other two objectives on the mean forecast data.}
\label{tab:diff_obj_actual}
\end{table}

\begin{table}[h]
\centering
\scalebox{0.8}{
\begin{tabular}{|c|c|c| c|}
    \hline
      \textbf{Objective}& \textbf{Algorithm} & \multicolumn{2}{|c|}{\textbf{Savings}} \\\cline{3-4}
     & & Cost & Carbon \\ 
     & &  (in EUR) &  (in gCO2eq)\\ \hline
     Cost  & DQN & 85177.23 & -82077.83  \\
     Optimization & MILP & \textbf{88198.84} & -43539.75  \\ \hline
     Carbon  & DQN& -36437.6 & 140219.63\\
     Optimization & MILP& -6016.38 & \textbf{163336.50}  \\ \hline
     Joint  & DQN & 24902.34& 92623.95 \\
     Optimization($\alpha=1.155$) &MILP &  46272.44& 135897.29  \\ \hline
\end{tabular}
}
\caption{Savings across different Objectives when mean of previous 10 days' actual values are used as forecasts. Imp: We chose $\alpha$ from the pareto optimal points in the further plot to compare apples to apples}
\label{tab:diff_obj_mean}
\end{table}

%Forecast values
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[p]
% \begin{tabular}{|c|cc|cc|cc|}
% \hline
% Forecast Method & \multicolumn{2}{c|}{Forecasting MAE} & \multicolumn{2}{c|}{Cost Savings()}                         & \multicolumn{2}{c|}{Carbon Emission Savings()}               \\
%                 & Price                       & Carbon & MILP                                   & DQN                & MILP                                    & DQN                \\ \hline
% Accurate        & \multicolumn{1}{c|}{0}      & 0      & \multicolumn{1}{c|}{116106.74}         & \textbf{117727.62} & \multicolumn{1}{c|}{\textbf{227272.49}} & 211594.86          \\ \hline
% Noise           & \multicolumn{1}{c|}{19.82}  & 19.08  & \multicolumn{1}{c|}{44635.65}          & \textbf{57858.85}  & \multicolumn{1}{c|}{123925.95}          & \textbf{163173.32} \\ \hline
% Yesterday       & \multicolumn{1}{c|}{9.70}   & 42.19  & \multicolumn{1}{c|}{77741.11}          & \textbf{83082.03}  & \multicolumn{1}{c|}{\textbf{138384.81}} & 129370.50          \\ \hline
% Mean            & \multicolumn{1}{c|}{9.94}   & 48.13  & \multicolumn{1}{c|}{\textbf{88198.84}} & 83241.51           & \multicolumn{1}{c|}{\textbf{163336.50}} & 135064.80          \\ \hline
% LightGBM        & \multicolumn{1}{c|}{11.88}  & 38.33  & \multicolumn{1}{c|}{55887.89}          & \textbf{62139.03}  & \multicolumn{1}{c|}{124398.81}          & \textbf{128731.44} \\ \hline
% N-BEATS         & \multicolumn{1}{c|}{10.13}  & 38.49  & \multicolumn{1}{c|}{73301.49}          & \textbf{76709.88}  & \multicolumn{1}{c|}{\textbf{145820.70}} & 130938.93          \\ \hline
% \end{tabular}
% \caption{Savings from two best performing algorithms: MILP and DQN to optimize cost and carbon savings. Takeaway: DQN performs well on low-intermediate error, on high error }
% \end{table}

\begin{table*}[hbtp]
\caption{Cost and carbon savings of two optimizers on different forecasting methods, each with varying mean average error(MAE).}
\scalebox{0.8}{
\begin{tabular}{|c|cc|cc|cc|}
\hline
Forecast Method & \multicolumn{2}{c|}{Forecasting MAE} & \multicolumn{2}{c|}{Cost Savings(K)}                 & \multicolumn{2}{c|}{Carbon Emission Savings($kgCO_2eq$)}     \\ \cline{2-7} 
                & \multicolumn{1}{c|}{Price}  & Carbon & \multicolumn{1}{c|}{MILP}          & DQN             & \multicolumn{1}{c|}{MILP}             & DQN             \\ \hline
Accurate        & \multicolumn{1}{c|}{0}      & 0      & \multicolumn{1}{c|}{116.1}         & \textbf{117.73} & \multicolumn{1}{c|}{\textbf{227.27}}  & 211.59          \\ \hline
Noise           & \multicolumn{1}{c|}{19.82}  & 19.08  & \multicolumn{1}{c|}{44.64}         & \textbf{57.86}  & \multicolumn{1}{c|}{123.93}           & \textbf{163.17} \\ \hline
Yesterday       & \multicolumn{1}{c|}{9.70}   & 42.19  & \multicolumn{1}{c|}{77.74}         & \textbf{83.08}  & \multicolumn{1}{c|}{\textbf{138.384}} & 129.37          \\ \hline
Mean            & \multicolumn{1}{c|}{9.94}   & 48.13  & \multicolumn{1}{c|}{\textbf{88.2}} & 83.24           & \multicolumn{1}{c|}{\textbf{163.34}}  & 135.06          \\ \hline
LightGBM        & \multicolumn{1}{c|}{11.88}  & 38.33  & \multicolumn{1}{c|}{55.89}         & \textbf{62.14}  & \multicolumn{1}{c|}{124.4}            & \textbf{128.73} \\ \hline
N-BEATS         & \multicolumn{1}{c|}{10.13}  & 38.49  & \multicolumn{1}{c|}{73.3}          & \textbf{76.71}  & \multicolumn{1}{c|}{\textbf{145.82}}  & 130.94          \\ \hline
\end{tabular}
}
\label{tab:milp_dqn_for_forecasts_ba}
\end{table*}

